Accretive Computation of Global Transformations

Global transformations form a categorical framework adapting graph transformations to describe fully synchronous rule systems on a given data structure.In this work we focus on data structures that can be captured as presheaves and study the computational aspects of such synchronous rule systems.To obtain an online algorithm, a complete study of the sub-steps within each synchronous step is done at the semantic level.This leads to the definition of accretive rule systems and a local criterion to characterize these systems.Finally an online computation algorithm for theses systems is given.

==> sierpinsky-common-v2.tex <==
\newcommand{\tri}[5]{
    \node[fill,circle,scale=0.3*(#4*#5*2)] (t0) at (#1,#2) {};
    \node[fill,circle,scale=0.3*(#4*#5*2)] (t1) at (#1+4,#2) {};
    \node[fill,circle,scale=0.3*(#4*#5*2)] (t2) at (#1+2,#2+6) {};
    \ifthenelse{\equal{#3}{0}}{
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (t0) edge (t1);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (t1) edge (t2);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (t0) edge (t2);
    }{\ifthenelse{\equal{#3}{1}}{
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (t0) edge (t1);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (t2) edge (t1);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (t2) edge (t0);
    }{
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (t1) edge (t0);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (t1) edge (t2);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (t2) edge (t0);
    }}
}

\newcommand{\edges}[5]{
    \node[fill,circle,scale=0.3*(#4*#5*2)] (e0) at (#1,#2-2) {};
    \node[fill,circle,scale=0.3*(#4*#5*2)] (e1) at (#1+4,#2-2) {};
    \node[fill,circle,scale=0.3*(#4*#5*2)] (e2) at (#1+5,#2+1) {};
    \node[fill,circle,scale=0.3*(#4*#5*2)] (e3) at (#1+3,#2+7) {};
    \node[fill,circle,scale=0.3*(#4*#5*2)] (e4) at (#1+1,#2+7) {};
    \node[fill,circle,scale=0.3*(#4*#5*2)] (e5) at (#1-1,#2+1) {};
    \ifthenelse{\equal{#3}{0}}{
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (e0) edge (e1);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (e2) edge (e3);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (e5) edge (e4);
    }{\ifthenelse{\equal{#3}{1}}{
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (e0) edge (e1);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (e3) edge (e2);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (e4) edge (e5);
    }{
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (e1) edge (e0);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (e2) edge (e3);
        \draw [shorten >=3*#4,shorten <=3*#4, ->] (e4) edge (e5);
    }}
}

\newcommand{\eedges}[4]{
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e0) at (#1,#2-2) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e01) at (#1+2,#2-2) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e1) at (#1+4,#2-2) {};
    
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e2) at (#1+5,#2+1) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e23) at (#1+4,#2+4) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e3) at (#1+3,#2+7) {};
    
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e4) at (#1+1,#2+7) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e45) at (#1,#2+4) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e5) at (#1-1,#2+1) {};
    
    \draw [shorten >=3*#3,shorten <=3*#3, ->] (e0) edge (e01);
    \draw [shorten >=3*#3,shorten <=3*#3, ->] (e1) edge (e01);
    
    \draw [shorten >=3*#3,shorten <=3*#3, ->] (e2) edge (e23);
    \draw [shorten >=3*#3,shorten <=3*#3, ->] (e3) edge (e23);
    
    \draw [shorten >=3*#3,shorten <=3*#3, ->] (e4) edge (e45);
    \draw [shorten >=3*#3,shorten <=3*#3, ->] (e5) edge (e45);
}

\newcommand{\nod}[4]{
    \node[fill,circle,scale=0.3*(#3*#4*2)] (n0) at (#1,#2) {};
}

\newcommand{\edge}[4]{
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e0) at (#1,#2) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e1) at (#1+4,#2) {};
    \draw [shorten >=3*#3,shorten <=3*#3, ->] (e0) edge (e1);
}

\newcommand{\eedge}[4]{
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e0) at (#1,#2) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e01) at (#1+2,#2) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (e1) at (#1+4,#2) {};
    \draw [shorten >=3*#3,shorten <=3*#3, ->] (e0) edge (e01);
    \draw [shorten >=3*#3,shorten <=3*#3, ->] (e1) edge (e01);
}

\newcommand{\nodes}[4] {
    \node[fill,circle,scale=0.3*(#3*#4*2)] (n0) at (#1-1.5,#2-1.5) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (n1) at (#1+5.5,#2-1.5) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (n2) at (#1+2,#2+9) {};
}

\newcommand{\boxes}[3]{
    \draw [color=gray, rounded corners=5*#3] (#1-0.5,#2-0.5) -- (#1+4.5,#2-0.5) -- (#1+2,#2+7) --cycle;

    \draw [color=gray, rounded corners=5*#3] (#1-0.25,#2-1.5) -- (#1+4.25,#2-1.5) -- (#1+4.25,#2-2.5) -- (#1-0.25,#2-2.5) --cycle;

    \draw [color=gray, rounded corners=5*#3] (#1+5-0.125, #2+1-0.625) -- (#1+3-0.375, #2+7+0.125) -- (#1+3+0.125, #2+7+0.625) -- (#1+5+0.375, #2+1-0.125) --cycle;
    
    \draw [color=gray, rounded corners=5*#3] (#1-1-0.375, #2+1-0.125) -- (#1+1-0.125, #2+7+0.625) -- (#1+1+0.375, #2+7+0.125) -- (#1-1+0.125, #2+1-0.625) --cycle;
    
    \draw [color=gray] (n0) circle (1/3.5 and 1.73/3.5);
    \draw [color=gray] (n1) circle (1/3.5 and 1.73/3.5);
    \draw [color=gray] (n2) circle (1/3.5 and 1.73/3.5);
}

\newcommand{\arrows}[1]{
    \draw let \p{e0}=(e0), \p{e1}=(e1), \p{t0}=(t0), \p{t1}=(t1) in
    [>=stealth, color=blue, thick, shorten >=10*#1,shorten <=10*#1, ->]
    (\x{e0}/2+\x{e1}/2, \y{e0}) -> (\x{t0}/2+\x{t1}/2, \y{t0});
    
    \draw let \p{e0}=(e2), \p{e1}=(e3), \p{t0}=(t1), \p{t1}=(t2) in
    [>=stealth, color=blue, thick, shorten >=10*#1,shorten <=10*#1, ->]
    (\x{e0}/2+\x{e1}/2, \y{e0}/2+\y{e1}/2) -> (\x{t0}/2+\x{t1}/2, \y{t0}/2+\y{t1}/2);
    
    \draw let \p{e0}=(e4), \p{e1}=(e5), \p{t0}=(t2), \p{t1}=(t0) in
    [>=stealth, color=blue, thick, shorten >=10*#1,shorten <=10*#1, ->]
    (\x{e0}/2+\x{e1}/2, \y{e0}/2+\y{e1}/2) -> (\x{t0}/2+\x{t1}/2, \y{t0}/2+\y{t1}/2);
    
    \draw [>=stealth, color=red, thick, shorten >=10*#1,shorten <=10*#1, ->] (n0) -> (e5);
    \draw [color=red, thick, shorten >=10*#1,shorten <=10*#1, ->] (n0) -> (e0);
    
    \draw [>=stealth, color=red, thick, shorten >=10*#1,shorten <=10*#1, ->] (n1) -> (e1);
    \draw [>=stealth, color=red, thick, shorten >=10*#1,shorten <=10*#1, ->] (n1) -> (e2);
    
    \draw [>=stealth, color=red, thick, shorten >=10*#1,shorten <=10*#1, ->] (n2) -> (e3);
    \draw [>=stealth, color=red, thick, shorten >=10*#1,shorten <=10*#1, ->] (n2) -> (e4);
}

\newcommand{\ttri}[4]{
    \begin{scope}[shift={(#1,#2)},scale=0.5]
        \tri{0}{0}{0}{#3}{#4}
        \tri{2}{6}{1}{#3}{#4}
        \tri{4}{0}{2}{#3}{#4}
    \end{scope}
    \node[fill,circle,scale=0.3*(#3*#4*2)] (t0) at (#1,#2) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (t1) at (#1+4,#2) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (t2) at (#1+2,#2+6) {};
}

\newcommand{\tttri}[4]{
    \begin{scope}[shift={(#1,#2)},scale=0.5]
        \ttri{0}{0}{#3}{#4}
        \ttri{2}{6}{#3}{#4}
        \ttri{4}{0}{#3}{#4}
    \end{scope}
    \node[fill,circle,scale=0.3*(#3*#4*2)] (t0) at (#1,#2) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (t1) at (#1+4,#2) {};
    \node[fill,circle,scale=0.3*(#3*#4*2)] (t2) at (#1+2,#2+6) {};
}

\newcommand{\dtttri}[4]{
    \ttri{0}{0}{#3}{#4}
    \eedges{0}{0}{#3}{#4}
    \nodes{0}{0}{#3}{#4}
    \boxes{0}{0}{#3}
    \arrows{#3}
    
    \ttri{3.5}{10.5}{#3}{#4}
    \eedges{3.5}{10.5}{#3}{#4}
    \nodes{3.5}{10.5}{#3}{#4}
    \boxes{3.5}{10.5}{#3}
    \arrows{#3}
    
    \ttri{7}{0}{#3}{#4}
    \eedges{7}{0}{#3}{#4}
    \nodes{7}{0}{#3}{#4}
    \boxes{7}{0}{#3}
    \arrows{#3}
}

\newcommand{\dttri}[4]{
    \tri{0}{0}{0}{#3}{#4}
    \edges{0}{0}{0}{#3}{#4}
    \nodes{0}{0}{#3}{#4}
    \boxes{0}{0}{#3}
    \arrows{#3}
    
    \tri{3.5}{10.5}{1}{#3}{#4}
    \edges{3.5}{10.5}{1}{#3}{#4}
    \nodes{3.5}{10.5}{#3}{#4}
    \boxes{3.5}{10.5}{#3}
    \arrows{#3}
    
    \tri{7}{0}{2}{#3}{#4}
    \edges{7}{0}{2}{#3}{#4}
    \nodes{7}{0}{#3}{#4}
    \boxes{7}{0}{#3}
    \arrows{#3}
}


